Leveraging Constraint Violation Signals For Action-Constrained Reinforcement Learning

In many RL applications, ensuring an agent's actions adhere to constraints is crucial for safety. Most previous methods in Action-Constrained Reinforcement Learning (ACRL) employ a projection layer after the policy network to correct the action. However projection-based methods suffer from issues like the zero gradient problem and higher runtime due to the usage of optimization solvers. Recently methods were proposed to train generative models to learn a differentiable mapping between latent variables and feasible actions to address this issue. However, generative models require training using samples from the constrained action space, which itself is challenging. To address such limitations, first, we define a target distribution for feasible actions based on constraint violation signals, and train normalizing flows by minimizing the KL divergence between an approximated distribution over feasible actions and the target. This eliminates the need to generate feasible action samples, greatly simplifying the flow model learning. Second, we integrate the learned flow model with existing deep RL methods, which restrict it to exploring only the feasible action space. Third, we extend our approach beyond ACRL to handle state-wise constraints by learning the constraint violation signal from the environment. Empirically, our approach has significantly fewer constraint violations while achieving similar or better quality in several control tasks than previous best methods.

==> reproducibility_checklist.tex <==
\section{Reproducibility Checklist}
This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced : yes
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results : yes
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper:~yes
\end{itemize}

\noindent Does this paper make theoretical contributions? yes

\noindent If yes, please complete the list below.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. : yes
\item All novel claims are stated formally (e.g., in theorem statements). : yes %(yes/partial/no)
\item Proofs of all novel claims are included. : yes % (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. : yes % (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. : yes % (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. : yes % (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. : NA % (yes/no/NA)
\end{itemize}

\noindent Does this paper rely on one or more datasets? no % (yes/no)

\noindent If yes, please complete the list below.

\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets : NA % (yes/partial/no/NA)
\item All novel datasets introduced in this paper are included in a data appendix. : NA % (yes/partial/no/NA)
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. : NA % (yes/partial/no/NA)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. : NA % (yes/no/NA)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. : NA % (yes/partial/no/NA)
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. : NA% (yes/partial/no/NA)
\end{itemize}


\noindent Does this paper include computational experiments? yes % (yes/no)

\noindent If yes, please complete the list below.


\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. : partial % (yes/partial/no).
\item All source code required for conducting and analyzing the experiments is included in a code appendix. : partial % (yes/partial/no)
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. : yes % (yes/partial/no)
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from : partial % (yes/partial/no)
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. : partial % (yes/partial/no/NA)
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. : partial % (yes/partial/no)
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. : yes % (yes/partial/no)
\item This paper states the number of algorithm runs used to compute each reported result. : yes % (yes/no)
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. : yes % (yes/no)
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). : no % (yes/partial/no)
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. : yes % (yes/partial/no/NA)
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. : partial % (yes/partial/no/NA)
\end{itemize}


